Relative hyperbolicity of ascending HNN extension of groups

We prove that for a finitely generated group G with a free factor system and an injective endomorphism that preserves the free factor system, the ascending HNN extension of G is hyperbolic relative to a collection of maximal parabolic subgroups. As a corollary, we see that if an injective endomorphism of a finite rank free group F is exponentially growing, the ascending HNN extension of F is relatively hyperbolic.

==> Combi.tex <==
@article {JWA1,
	AUTHOR = {Anderson, James W.},
	TITLE = {Intersections of analytically and geometrically finite
		subgroups of {K}leinian groups},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {343},
	YEAR = {1994},
	NUMBER = {1},
	PAGES = {87--98},
	ISSN = {0002-9947},
	MRCLASS = {30F40 (57M50)},
	MRNUMBER = {1207578},
	MRREVIEWER = {Ara Basmajian},
	DOI = {10.2307/2154522},
	URL = {https://doi.org/10.2307/2154522},
}
@article {JWA2,
	AUTHOR = {Anderson, James W.},
	TITLE = {Intersections of topologically tame subgroups of {K}leinian
		groups},
	JOURNAL = {J. Anal. Math.},
	FJOURNAL = {Journal d'Analyse Math\'{e}matique},
	VOLUME = {65},
	YEAR = {1995},
	PAGES = {77--94},
	ISSN = {0021-7670},
	MRCLASS = {30F40 (20H10)},
	MRNUMBER = {1335369},
	MRREVIEWER = {C. Maclachlan},
	DOI = {10.1007/BF02788766},
	URL = {https://doi.org/10.1007/BF02788766},
}
@article {JWA3,
	AUTHOR = {Anderson, James W.},
	TITLE = {The limit set intersection theorem for finitely generated
		{K}leinian groups},
	JOURNAL = {Math. Res. Lett.},
	FJOURNAL = {Mathematical Research Letters},
	VOLUME = {3},
	YEAR = {1996},
	NUMBER = {5},
	PAGES = {675--692},
	ISSN = {1073-2780},
	MRCLASS = {30F40 (20H10)},
	MRNUMBER = {1418580},
	MRREVIEWER = {R. A. Hidalgo},
	DOI = {10.4310/MRL.1996.v3.n5.a9},
	URL = {https://doi.org/10.4310/MRL.1996.v3.n5.a9},
}
@article {JWA4,
	AUTHOR = {Anderson, James W.},
	TITLE = {Limit set intersection theorems for {K}leinian groups and a
		conjecture of {S}usskind},
	JOURNAL = {Comput. Methods Funct. Theory},
	FJOURNAL = {Computational Methods and Function Theory},
	VOLUME = {14},
	YEAR = {2014},
	NUMBER = {2-3},
	PAGES = {453--464},
	ISSN = {1617-9447},
	MRCLASS = {30F40 (20H10 37F30 57M50)},
	MRNUMBER = {3265372},
	MRREVIEWER = {Yasushi Yamashita},
	DOI = {10.1007/s40315-014-0078-7},
	URL = {https://doi.org/10.1007/s40315-014-0078-7},
}
@article {b-r,
	AUTHOR = {Baker, O. and Riley, T. R.},
	TITLE = {Cannon-{T}hurston maps do not always exist},
	JOURNAL = {Forum Math. Sigma},
	FJOURNAL = {Forum of Mathematics. Sigma},
	VOLUME = {1},
	YEAR = {2013},
	PAGES = {e3, 11},
	MRCLASS = {20F67 (20F65 57M07)},
	MRNUMBER = {3143716},
	MRREVIEWER = {Jos\'{e} Burillo},
	DOI = {10.1017/fms.2013.4},
	URL = {https://doi.org/10.1017/fms.2013.4},
}
@article {rs,
	AUTHOR = {Riley, Tim R. and Sale, Andrew W.},
	TITLE = {Palindromic width of wreath products, metabelian groups, and
		max-n solvable groups},
	JOURNAL = {Groups Complex. Cryptol.},
	FJOURNAL = {Groups. Complexity. Cryptology},
	VOLUME = {6},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {121--132},
	ISSN = {1867-1144},
	MRCLASS = {20F16 (20F65)},
	MRNUMBER = {3276196},
	MRREVIEWER = {Vitaly A. Roman\cprime kov},
	DOI = {10.1515/gcc-2014-0009},
	URL = {https://doi.org/10.1515/gcc-2014-0009},
}
@article {CT,
	AUTHOR = {Cannon, James W. and Thurston, William P.},
	TITLE = {Group invariant {P}eano curves},
	JOURNAL = {Geom. Topol.},
	FJOURNAL = {Geometry \& Topology},
	VOLUME = {11},
	YEAR = {2007},
	PAGES = {1315--1355},
	ISSN = {1465-3060},
	MRCLASS = {57M50 (57M07)},
	MRNUMBER = {2326947},
	MRREVIEWER = {Darryl McCullough},
	DOI = {10.2140/gt.2007.11.1315},
	URL = {https://doi.org/10.2140/gt.2007.11.1315},
}
@article {MjReeves,
	AUTHOR = {Mj, Mahan and Reeves, Lawrence},
	TITLE = {A combination theorem for strong relative hyperbolicity},
	JOURNAL = {Geom. Topol.},
	FJOURNAL = {Geometry \& Topology},
	VOLUME = {12},
	YEAR = {2008},
	NUMBER = {3},
	PAGES = {1777--1798},
	ISSN = {1465-3060},
	MRCLASS = {20F67 (57M50)},
	MRNUMBER = {2421140},
	DOI = {10.2140/gt.2008.12.1777},
	URL = {https://doi.org/10.2140/gt.2008.12.1777},
}
@article {SusSwa,
	AUTHOR = {Susskind, Perry and Swarup, Gadde A.},
	TITLE = {Limit sets of geometrically finite hyperbolic groups},
	JOURNAL = {Amer. J. Math.},
	FJOURNAL = {American Journal of Mathematics},
	VOLUME = {114},
	YEAR = {1992},
	NUMBER = {2},
	PAGES = {233--250},
	ISSN = {0002-9327},
	MRCLASS = {57S30 (20F32 30F40)},
	MRNUMBER = {1156565},
	MRREVIEWER = {Boris N. Apanasov},
	DOI = {10.2307/2374703},
	URL = {https://doi.org/10.2307/2374703},
}
@article {MjPal,
	AUTHOR = {Mj, Mahan and Pal, Abhijit},
	TITLE = {Relative hyperbolicity, trees of spaces and
		{C}annon-{T}hurston maps},
	JOURNAL = {Geom. Dedicata},
	FJOURNAL = {Geometriae Dedicata},
	VOLUME = {151},
	YEAR = {2011},
	PAGES = {59--78},
	ISSN = {0046-5755},
	MRCLASS = {20F65 (57M50)},
	MRNUMBER = {2780738},
	MRREVIEWER = {Vassilis Metaftsis},
	DOI = {10.1007/s10711-010-9519-2},
	URL = {https://doi.org/10.1007/s10711-010-9519-2},
}
@article {Pal,
	AUTHOR = {Pal, Abhijit},
	TITLE = {Relatively hyperbolic extensions of groups and
		{C}annon-{T}hurston maps},
	JOURNAL = {Proc. Indian Acad. Sci. Math. Sci.},
	FJOURNAL = {Indian Academy of Sciences. Proceedings. Mathematical
		Sciences},
	VOLUME = {120},
	YEAR = {2010},
	NUMBER = {1},
	PAGES = {57--68},
	ISSN = {0253-4142},
	MRCLASS = {20F67 (57M50)},
	MRNUMBER = {2654898},
	MRREVIEWER = {Mahan Mj},
	DOI = {10.1007/s12044-010-0009-0},
	URL = {https://doi.org/10.1007/s12044-010-0009-0},
}
@article {pranab,
	AUTHOR = {Mj, Mahan and Sardar, Pranab},
	TITLE = {A combination theorem for metric bundles},
	JOURNAL = {Geom. Funct. Anal.},
	FJOURNAL = {Geometric and Functional Analysis},
	VOLUME = {22},
	YEAR = {2012},
	NUMBER = {6},
	PAGES = {1636--1707},
	ISSN = {1016-443X},
	MRCLASS = {20F65 (57M50)},
	MRNUMBER = {3000500},
	MRREVIEWER = {Sylvain Maillot},
	DOI = {10.1007/s00039-012-0196-1},
	URL = {https://doi.org/10.1007/s00039-012-0196-1},
}
@article {PS,
	AUTHOR = {Sardar, Pranab},
	TITLE = {Graphs of hyperbolic groups and a limit set intersection
		theorem},
	JOURNAL = {Proc. Amer. Math. Soc.},
	FJOURNAL = {Proceedings of the American Mathematical Society},
	VOLUME = {146},
	YEAR = {2018},
	NUMBER = {5},
	PAGES = {1859--1871},
	ISSN = {0002-9939},
	MRCLASS = {20F67},
	MRNUMBER = {3767341},
	MRREVIEWER = {Alessandro Sisto},
	DOI = {10.1090/proc/13871},
	URL = {https://doi.org/10.1090/proc/13871},
}
@book {Sus,
	AUTHOR = {Susskind, Perry Douglas},
	TITLE = {O{n} {Kleinian} {groups} {with} {intersecting} {limit} {sets}},
	NOTE = {Thesis (Ph.D.)--State University of New York at Stony Brook},
	PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
	YEAR = {1982},
	PAGES = {59},
	MRCLASS = {Thesis},
	MRNUMBER = {2632000},
	URL =
	{http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:8217714},
}
@article {mit1,
	AUTHOR = {Mitra, Mahan},
	TITLE = {Cannon-{T}hurston maps for hyperbolic group extensions},
	JOURNAL = {Topology},
	FJOURNAL = {Topology. An International Journal of Mathematics},
	VOLUME = {37},
	YEAR = {1998},
	NUMBER = {3},
	PAGES = {527--538},
	ISSN = {0040-9383},
	MRCLASS = {57M07 (20F32 57M10)},
	MRNUMBER = {1604882},
	MRREVIEWER = {Sadayoshi Kojima},
	DOI = {10.1016/S0040-9383(97)00036-0},
	URL = {https://doi.org/10.1016/S0040-9383(97)00036-0},
}


@article {mit0,
	AUTHOR = {Mitra, Mahan},
	TITLE = {Cannon-{T}hurston maps for trees of hyperbolic metric spaces},
	JOURNAL = {J. Differential Geom.},
	FJOURNAL = {Journal of Differential Geometry},
	VOLUME = {48},
	YEAR = {1998},
	NUMBER = {1},
	PAGES = {135--164},
	ISSN = {0022-040X},
	MRCLASS = {57M07 (20F32 57M50)},
	MRNUMBER = {1622603},
	MRREVIEWER = {Michah Sageev},
	URL = {http://projecteuclid.org/euclid.jdg/1214460609},
}
@article {mj1,
	AUTHOR = {Mj, Mahan},
	TITLE = {Cannon-{T}hurston maps for surface groups},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {179},
	YEAR = {2014},
	NUMBER = {1},
	PAGES = {1--80},
	ISSN = {0003-486X},
	MRCLASS = {57M50 (20F65 20H10 30F40)},
	MRNUMBER = {3126566},
	MRREVIEWER = {James W. Anderson},
	DOI = {10.4007/annals.2014.179.1.1},
	URL = {https://doi.org/10.4007/annals.2014.179.1.1},
}
@article {bbg,
	AUTHOR = {Bardakov, Valeriy G. and Bryukhanov, Oleg V. and Gongopadhyay,
		Krishnendu},
	TITLE = {Palindromic widths of nilpotent and wreath products},
	JOURNAL = {Proc. Indian Acad. Sci. Math. Sci.},
	FJOURNAL = {Indian Academy of Sciences. Proceedings. Mathematical
		Sciences},
	VOLUME = {127},
	YEAR = {2017},
	NUMBER = {1},
	PAGES = {99--108},
	ISSN = {0253-4142},
	MRCLASS = {20F16 (20E22)},
	MRNUMBER = {3605244},
	MRREVIEWER = {Andrei Smolensky},
	DOI = {10.1007/s12044-016-0296-1},
	URL = {https://doi.org/10.1007/s12044-016-0296-1},
}
@article {bg1,
	AUTHOR = {Bardakov, Valeriy G. and Gongopadhyay, Krishnendu},
	TITLE = {Palindromic width of free nilpotent groups},
	JOURNAL = {J. Algebra},
	FJOURNAL = {Journal of Algebra},
	VOLUME = {402},
	YEAR = {2014},
	PAGES = {379--391},
	ISSN = {0021-8693},
	MRCLASS = {20F18 (20D15 20E05)},
	MRNUMBER = {3160428},
	MRREVIEWER = {Martin Edjvet},
	DOI = {10.1016/j.jalgebra.2013.12.002},
	URL = {https://doi.org/10.1016/j.jalgebra.2013.12.002},
}


@article {bg2,
	AUTHOR = {Bardakov, Valeriy G. and Gongopadhyay, Krishnendu},
	TITLE = {On palindromic width of certain extensions and quotients of
		free nilpotent groups},
	JOURNAL = {Internat. J. Algebra Comput.},
	FJOURNAL = {International Journal of Algebra and Computation},
	VOLUME = {24},
	YEAR = {2014},
	NUMBER = {5},
	PAGES = {553--567},
	ISSN = {0218-1967},
	MRCLASS = {20F18},
	MRNUMBER = {3254714},
	MRREVIEWER = {Gunnar Traustason},
	DOI = {10.1142/S0218196714500246},
	URL = {https://doi.org/10.1142/S0218196714500246},
}


@article {bgs,
	AUTHOR = {Bardakov, Valeriy G. and Gongopadhyay, Krishnendu and Singh,
		Mahender},
	TITLE = {Palindromic automorphisms of free groups},
	JOURNAL = {J. Algebra},
	FJOURNAL = {Journal of Algebra},
	VOLUME = {438},
	YEAR = {2015},
	PAGES = {260--282},
	ISSN = {0021-8693},
	MRCLASS = {20F28 (20E05)},
	MRNUMBER = {3353032},
	MRREVIEWER = {H. Heineken},
	DOI = {10.1016/j.jalgebra.2015.05.014},
	URL = {https://doi.org/10.1016/j.jalgebra.2015.05.014},
}


@article {BG-solv,
	AUTHOR = {Bardakov, Valeriy G. and Gongopadhyay, Krishnendu},
	TITLE = {Palindromic width of finitely generated solvable groups},
	JOURNAL = {Comm. Algebra},
	FJOURNAL = {Communications in Algebra},
	VOLUME = {43},
	YEAR = {2015},
	NUMBER = {11},
	PAGES = {4809--4824},
	ISSN = {0092-7872},
	MRCLASS = {20F16 (20E22 20F05)},
	MRNUMBER = {3422368},
	MRREVIEWER = {T. O. Hawkes},
	DOI = {10.1080/00927872.2014.952738},
	URL = {https://doi.org/10.1080/00927872.2014.952738},
}


@article {vw,
	AUTHOR = {Bardakov, V. and Gongopadhyay, K. and Singh, M. and Vesnin, A.
		and Wu, J.},
	TITLE = {Some problems on knots, braids, and automorphism groups},
	JOURNAL = {Sib. \`Elektron. Mat. Izv.},
	FJOURNAL = {Sibirskie \`Elektronnye Matematicheskie Izvestiya. Siberian
		Electronic Mathematical Reports},
	VOLUME = {12},
	YEAR = {2015},
	PAGES = {394--405},
	MRCLASS = {57M25},
	MRNUMBER = {3493780},
	MRREVIEWER = {Seiichi Kamada},
}
@article {bst,
	AUTHOR = {Bardakov, Valery and Shpilrain, Vladimir and Tolstykh,
		Vladimir},
	TITLE = {On the palindromic and primitive widths of a free group},
	JOURNAL = {J. Algebra},
	FJOURNAL = {Journal of Algebra},
	VOLUME = {285},
	YEAR = {2005},
	NUMBER = {2},
	PAGES = {574--585},
	ISSN = {0021-8693},
	MRCLASS = {20E05},
	MRNUMBER = {2125453},
	MRREVIEWER = {Waldemar M. Ho\l ubowski},
	DOI = {10.1016/j.jalgebra.2004.11.003},
	URL = {https://doi.org/10.1016/j.jalgebra.2004.11.003},
}


@article {bt,
	AUTHOR = {Bardakov, Valery and Tolstykh, Vladimir},
	TITLE = {The palindromic width of a free product of groups},
	JOURNAL = {J. Aust. Math. Soc.},
	FJOURNAL = {Journal of the Australian Mathematical Society},
	VOLUME = {81},
	YEAR = {2006},
	NUMBER = {2},
	PAGES = {199--208},
	ISSN = {1446-7887},
	MRCLASS = {20E06 (20F05)},
	MRNUMBER = {2267791},
	MRREVIEWER = {Martin Edjvet},
	DOI = {10.1017/S1446788700015822},
	URL = {https://doi.org/10.1017/S1446788700015822},
}
@article {bf,
	AUTHOR = {Bestvina, M. and Feighn, M.},
	TITLE = {A combination theorem for negatively curved groups},
	JOURNAL = {J. Differential Geom.},
	FJOURNAL = {Journal of Differential Geometry},
	VOLUME = {35},
	YEAR = {1992},
	NUMBER = {1},
	PAGES = {85--101},
	ISSN = {0022-040X},
	MRCLASS = {53C23 (57M50)},
	MRNUMBER = {1152226},
	MRREVIEWER = {Tadeusz Januszkiewicz},
	URL = {http://projecteuclid.org/euclid.jdg/1214447806},
}
@article {ft,
	AUTHOR = {Fink, Elisabeth and Thom, Andreas},
	TITLE = {Palindromic words in simple groups},
	JOURNAL = {Internat. J. Algebra Comput.},
	FJOURNAL = {International Journal of Algebra and Computation},
	VOLUME = {25},
	YEAR = {2015},
	NUMBER = {3},
	PAGES = {439--444},
	ISSN = {0218-1967},
	MRCLASS = {20E32 (20F69)},
	MRNUMBER = {3334644},
	MRREVIEWER = {Colva M. Roney-Dougal},
	DOI = {10.1142/S0218196715500046},
	URL = {https://doi.org/10.1142/S0218196715500046},
}
@article {f2,
	AUTHOR = {Fink, Elisabeth},
	TITLE = {Conjugacy growth and width of certain branch groups},
	JOURNAL = {Internat. J. Algebra Comput.},
	FJOURNAL = {International Journal of Algebra and Computation},
	VOLUME = {24},
	YEAR = {2014},
	NUMBER = {8},
	PAGES = {1213--1231},
	ISSN = {0218-1967},
	MRCLASS = {20F65 (20F69)},
	MRNUMBER = {3296364},
	MRREVIEWER = {Mustafa G\"{o}khan Benli},
	DOI = {10.1142/S0218196714500544},
	URL = {https://doi.org/10.1142/S0218196714500544},
}
@article {fink1,
	AUTHOR = {Fink, Elisabeth},
	TITLE = {Palindromic width of wreath products},
	JOURNAL = {J. Algebra},
	FJOURNAL = {Journal of Algebra},
	VOLUME = {471},
	YEAR = {2017},
	PAGES = {1--12},
	ISSN = {0021-8693},
	MRCLASS = {20E22 (20F05)},
	MRNUMBER = {3569177},
	MRREVIEWER = {Valeriy G. Bardakov},
	DOI = {10.1016/j.jalgebra.2016.09.015},
	URL = {https://doi.org/10.1016/j.jalgebra.2016.09.015},
}
@article {TDDS,
	AUTHOR = {Das, Tushar and Simmons, David.},
	TITLE = {Intersecting limit sets of Kleinian subgroups and Susskind’s question.},
	URL = {https://arxiv.org/pdf/1802.07654.pdf},
}
@article {Yang,
	AUTHOR = {Yang, Wen-yuan},
	TITLE = {Limit sets of relatively hyperbolic groups},
	JOURNAL = {Geom. Dedicata},
	FJOURNAL = {Geometriae Dedicata},
	VOLUME = {156},
	YEAR = {2012},
	PAGES = {1--12},
	ISSN = {0046-5755},
	MRCLASS = {20F67},
	MRNUMBER = {2863542},
	MRREVIEWER = {Shihai Yang},
	DOI = {10.1007/s10711-011-9586-z},
	URL = {https://doi.org/10.1007/s10711-011-9586-z},
}
@incollection {Pal3,
	AUTHOR = {Saarela, Aleksi},
	TITLE = {Palindromic length in free monoids and free groups},
	BOOKTITLE = {Combinatorics on words},
	SERIES = {Lecture Notes in Comput. Sci.},
	VOLUME = {10432},
	PAGES = {203--213},
	PUBLISHER = {Springer, Cham},
	YEAR = {2017},
	MRCLASS = {68R15 (20F10)},
	MRNUMBER = {3703625},
}
@article {mo,
	AUTHOR = {Matsuda, Yoshifumi and Oguni, Shin-ichi},
	TITLE = {On {C}annon-{T}hurston maps for relatively hyperbolic groups},
	JOURNAL = {J. Group Theory},
	FJOURNAL = {Journal of Group Theory},
	VOLUME = {17},
	YEAR = {2014},
	NUMBER = {1},
	PAGES = {41--47},
	ISSN = {1433-5883},
	MRCLASS = {57Rxx},
	MRNUMBER = {3176651},
	MRREVIEWER = {Mark F. Hagen},
	DOI = {10.1515/jgt-2013-0024},
	URL = {https://doi.org/10.1515/jgt-2013-0024},
}
@article {gk,
	AUTHOR = {Gilman, Jane and Keen, Linda},
	TITLE = {Discreteness criteria and the hyperbolic geometry of
		palindromes},
	JOURNAL = {Conform. Geom. Dyn.},
	FJOURNAL = {Conformal Geometry and Dynamics. An Electronic Journal of the
		American Mathematical Society},
	VOLUME = {13},
	YEAR = {2009},
	PAGES = {76--90},
	MRCLASS = {30F10 (20E05 30F45)},
	MRNUMBER = {2476657},
	MRREVIEWER = {Hiroshige Shiga},
	DOI = {10.1090/S1088-4173-09-00191-X},
	URL = {https://doi.org/10.1090/S1088-4173-09-00191-X},
}
@article {gj,
	AUTHOR = {Glover, Henry H. and Jensen, Craig A.},
	TITLE = {Geometry for palindromic automorphism groups of free groups},
	JOURNAL = {Comment. Math. Helv.},
	FJOURNAL = {Commentarii Mathematici Helvetici},
	VOLUME = {75},
	YEAR = {2000},
	NUMBER = {4},
	PAGES = {644--667},
	ISSN = {0010-2571},
	MRCLASS = {20F28 (20F65 20J05 55N91)},
	MRNUMBER = {1789180},
	MRREVIEWER = {Vincent Guirardel},
	DOI = {10.1007/s000140050143},
	URL = {https://doi.org/10.1007/s000140050143},
}
@article {ful,
	AUTHOR = {Fullarton, Neil J.},
	TITLE = {A generating set for the palindromic {T}orelli group},
	JOURNAL = {Algebr. Geom. Topol.},
	FJOURNAL = {Algebraic \& Geometric Topology},
	VOLUME = {15},
	YEAR = {2015},
	NUMBER = {6},
	PAGES = {3535--3567},
	ISSN = {1472-2747},
	MRCLASS = {20E36 (20E05 20F05 57M07)},
	MRNUMBER = {3450770},
	MRREVIEWER = {Michael L. Mihalik},
	DOI = {10.2140/agt.2015.15.3535},
	URL = {https://doi.org/10.2140/agt.2015.15.3535},
}
@article {ps-kap,
	AUTHOR = {Kapovich, Micheal and Sardar, Pranab},
	TITLE = {Hyperbolic trees of space II: Existence of Cannon-Thurston maps,},
}
@article {kgsk,
	AUTHOR = {Gongopadhyay, Krishnendu and Krishna, Swathi},
	TITLE = {Palindromic widths of graph of groups},
	JOURNAL = {Proc. Indian Acad. Sci. Math. Sci.},
	FJOURNAL = {Indian Academy of Sciences. Proceedings. Mathematical Sciences},
	VOLUME = {130},
	YEAR = {2020},
	NUMBER = {1},
	PAGES = {Paper No. 22, 15},
	ISSN = {0253-4142},
	DOI = {10.1007/s12044-019-0544-2} 
	URL = {https://doi.org/10.1007/s12044-019-0544-2},
}
@article {sk,
	AUTHOR = {Krishna, Swathi},
	TITLE = {A Limit Intersection Theorem for Graph of Relatively Hyperbolic Groups},
	JOURNAL = {Proc. Indian Acad. Sci. Math. Sci.},
	FJOURNAL = {Indian Academy of Sciences. Proceedings. Mathematical Sciences},
	VOLUME = {130},
	YEAR = {2020},
	NUMBER = {1},
	PAGES = {Paper No. 36, 18},
	ISSN = {0253-4142},
	MRCLASS = {20F65 (20E06)},
	MRNUMBER = {4067149},
	DOI = {10.1007/s12044-020-0563-z}
	URL = {https://doi.org/10.1007/s12044-020-0563-z},
}
@article {PS1,
	AUTHOR = {Sardar, Pranab},
	TITLE = {Corrigendum to ``Graphs of hyperbolic groups and a limit set intersection theorem''.},
	URL = {https://arxiv.org/abs/1909.01823},
}

@article {MR3126566,
	AUTHOR = {Mj, Mahan},
	TITLE = {Cannon-{T}hurston maps for surface groups},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {179},
	YEAR = {2014},
	NUMBER = {1},
	PAGES = {1--80},
	ISSN = {0003-486X},
	MRCLASS = {57M50 (20F65 20H10 30F40)},
	MRNUMBER = {3126566},
	MRREVIEWER = {James W. Anderson},
	DOI = {10.4007/annals.2014.179.1.1},
	URL = {https://doi.org/10.4007/annals.2014.179.1.1},
}
@book {bh,
	AUTHOR = {Bridson, Martin R. and Haefliger, Andr\'{e}},
	TITLE = {Metric spaces of non-positive curvature},
	SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
		Principles of Mathematical Sciences]},
	VOLUME = {319},
	PUBLISHER = {Springer-Verlag, Berlin},
	YEAR = {1999},
	PAGES = {xxii+643},
	ISBN = {3-540-64324-9},
	MRCLASS = {53C23 (20F65 53C70 57M07)},
	MRNUMBER = {1744486},
	MRREVIEWER = {Athanase Papadopoulos},
	DOI = {10.1007/978-3-662-12494-9},
	URL = {https://doi.org/10.1007/978-3-662-12494-9},
}
@article {lt,
	AUTHOR = {Lim, Seonhee and Thomas, Anne},
	TITLE = {Covering theory for complexes of groups},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {212},
	YEAR = {2008},
	NUMBER = {7},
	PAGES = {1632--1663},
	ISSN = {0022-4049},
	MRCLASS = {57M10 (20E42 57M07)},
	MRNUMBER = {2400734},
	MRREVIEWER = {Goulnara N. Arzhantseva},
	DOI = {10.1016/j.jpaa.2007.10.012},
	URL = {https://doi.org/10.1016/j.jpaa.2007.10.012},
}
@Article{bowditch-stacks,
	author = "B. H. Bowditch",
	title = "Stacks of hyperbolic spaces and ends of 3 manifolds",
	journal = "preprint, Southampton",
	year = "2002"
}
@Article{pssk,
	author = "Krishna, Swathi and Sardar, Pranab",
	title = "Pullbacks of metric bundles and {C}annon-{T}hurston maps",
	note= {\url{https://arxiv.org/pdf/2007.13109.pdf}}
	year = "2020"
}

@article{ct-conical,
	title = "Conical limit points and the cannon-thurston map",
	author = "Jeon, Woojin and Kapovich, Ilya and Leininger, Christopher and Ohshika, Ken'Ichi",
	year = "2016",
	doi = "10.1090/ecgd/294",
	language = "English (US)",
	volume = "20",
	pages = "58--80",
	journal = "Conformal Geometry and Dynamics",
	issn = "1088-4173",
	publisher = "American Mathematical Society",
	number = "4",
}
@article{kap-lus,
	author = {Kapovich, Ilya and Lustig, Martin},
	title = "{Cannon–Thurston fibers for iwip automorphisms of $F_N$}",
	journal = {Journal of the London Mathematical Society},
	volume = {91},
	number = {1},
	pages = {203-224},
	year = {2015},
	month = {01},
	issn = {0024-6107},
	doi = {10.1112/jlms/jdu069},
	url = {https://doi.org/10.1112/jlms/jdu069},
	eprint = {https://academic.oup.com/jlms/article-pdf/91/1/203/9683316/jdu069.pdf},
}
@article{mjlecuire,
	author = {Lecuire, Cyril and Mj, Mahan},
	title = "{Horospheres in Degenerate 3-Manifolds}",
	journal = {International Mathematics Research Notices},
	volume = {2018},
	number = {3},
	pages = {816-861},
	year = {2016},
	month = {12},
	issn = {1073-7928},
	doi = {10.1093/imrn/rnw256},
	url = {https://doi.org/10.1093/imrn/rnw256},
	eprint = {https://academic.oup.com/imrn/article-pdf/2018/3/816/23812399/rnw256.pdf},
}
@article{ger,
	author = { Gerasimov, Victor},
	title = "{Floyd maps for relatively hyperbolic groups}",
	journal = {Geometric and Functional Analysis},
	volume = {22},
	number = {5},
	pages = {1361-1399},
	year = {2012},
	issn = {1420-8970},
	doi = {10.1007/s00039-012-0175-6},
	url = {https://doi.org/10.1007/s00039-012-0175-6},
}
@Article{gromov,
	author = "M. Gromov",
	title = "Hyperbolic {G}roups",
	journal = "in Essays in Group Theory, ed. Gersten, MSRI Publ.,vol.8, Springer Verlag",
	year = "1987",
	pages = "75--263"
}
@Article{Field,
	author = "Field, Elizabeth",
	title = "Trees, dendrites, and the Cannon-Thurston map ",
	journal = "preprint",
	year = "2019"
}
@book{osin,
	title={Relatively Hyperbolic Groups: Intrinsic Geometry, Algebraic Properties, and Algorithmic Problems: Intrinsic Geometry, Algebraic Properties, and Algorithmic Problems},
	author={Osin, D.V.},
	isbn={9780821838211},
	lccn={2005053663},
	series={American Mathematical Society},
	url={https://books.google.co.in/books?id=tunUCQAAQBAJ},
	year={2006},
	publisher={American Mathematical Society}
}
@article {fh94,
	AUTHOR = {Fel'shtyn, Alexander and Hill, Richard},
	TITLE = {The {R}eidemeister zeta function with applications to
		{N}ielsen theory and a connection with {R}eidemeister torsion},
	JOURNAL = {$K$-Theory},
	FJOURNAL = {$K$-Theory. An Interdisciplinary Journal for the Development,
		Application, and Influence of $K$-Theory in the Mathematical
		Sciences},
	VOLUME = {8},
	YEAR = {1994},
	NUMBER = {4},
	PAGES = {367--393},
	ISSN = {0920-3036},
	MRCLASS = {57Q10 (55M20 58F20)},
	MRNUMBER = {1300546},
	MRREVIEWER = {Christopher K. McCord},
	DOI = {10.1007/BF00961408},
	URL = {https://doi.org/10.1007/BF00961408},
}
@article {fel01,
	AUTHOR = {Fel'shtyn, Alexander},
	TITLE = {The {R}eidemeister number of any automorphism of a {G}romov
		hyperbolic group is infinite},
	JOURNAL = {Zap. Nauchn. Sem. S.-Peterburg. Otdel. Mat. Inst. Steklov.
		(POMI)},
	FJOURNAL = {Rossi\u{\i}skaya Akademiya Nauk. Sankt-Peterburgskoe Otdelenie.
		Matematicheski\u{\i} Institut im. V. A. Steklova. Zapiski Nauchnykh
		Seminarov (POMI)},
	VOLUME = {279},
	YEAR = {2001},
	NUMBER = {Geom. i Topol. 6},
	PAGES = {229--240, 250},
	ISSN = {0373-2703},
	MRCLASS = {20F67 (20F28 37E30 57M07)},
	MRNUMBER = {1846083},
	MRREVIEWER = {Gilbert Levitt},
	DOI = {10.1023/B:JOTH.0000008749.42806.e3},
	URL = {https://doi.org/10.1023/B:JOTH.0000008749.42806.e3},
}
@article {ll00,
	AUTHOR = {Levitt, Gilbert and Lustig, Martin},
	TITLE = {Most automorphisms of a hyperbolic group have very simple
		dynamics},
	JOURNAL = {Ann. Sci. \'{E}cole Norm. Sup. (4)},
	FJOURNAL = {Annales Scientifiques de l'\'{E}cole Normale Sup\'{e}rieure. Quatri\`eme
		S\'{e}rie},
	VOLUME = {33},
	YEAR = {2000},
	NUMBER = {4},
	PAGES = {507--517},
	ISSN = {0012-9593},
	MRCLASS = {20F67 (20F28 20F65 37C85)},
	MRNUMBER = {1832822},
	MRREVIEWER = {Eric M. Freden},
	DOI = {10.1016/S0012-9593(00)00120-8},
	URL = {https://doi.org/10.1016/S0012-9593(00)00120-8},
}
@article {fg10,
	AUTHOR = {Fel'shtyn, Alexander and Gon\c{c}alves, Daciberg L.},
	TITLE = {Twisted conjugacy classes in symplectic groups, mapping class
		groups and braid groups},
	NOTE = {With an appendix written jointly with Francois Dahmani},
	JOURNAL = {Geom. Dedicata},
	FJOURNAL = {Geometriae Dedicata},
	VOLUME = {146},
	YEAR = {2010},
	PAGES = {211--223},
	ISSN = {0046-5755},
	MRCLASS = {20E45 (20F36 20F65 20G30 37C25 55M20 57M20)},
	MRNUMBER = {2644279},
	MRREVIEWER = {Darryl McCullough},
	DOI = {10.1007/s10711-009-9434-6},
	URL = {https://doi.org/10.1007/s10711-009-9434-6},
}
@article {dow-kap-taylor,
	AUTHOR = {Dowdall, Spencer and Kapovich, Ilya and Taylor, Samuel J.},
	TITLE = {Cannon-{T}hurston maps for hyperbolic free group extensions},
	JOURNAL = {Israel J. Math.},
	FJOURNAL = {Israel Journal of Mathematics},
	VOLUME = {216},
	YEAR = {2016},
	NUMBER = {2},
	PAGES = {753--797},
	ISSN = {0021-2172},
	MRCLASS = {20F65 (20E22 20F05 20F28 20F67 20F69 57M07 57M27)},
	MRNUMBER = {3557464},
	MRREVIEWER = {Dawid Kielak},
	DOI = {10.1007/s11856-016-1426-2},
	URL = {https://doi.org/10.1007/s11856-016-1426-2},
}
@article {mj-lam,
	AUTHOR = {Mj, Mahan},
	TITLE = {Ending laminations and {C}annon-{T}hurston maps},
	NOTE = {With an appendix by Shubhabrata Das and Mj},
	JOURNAL = {Geom. Funct. Anal.},
	FJOURNAL = {Geometric and Functional Analysis},
	VOLUME = {24},
	YEAR = {2014},
	NUMBER = {1},
	PAGES = {297--321},
	ISSN = {1016-443X},
	MRCLASS = {57M50 (20F65 20F67 22E40)},
	MRNUMBER = {3177384},
	MRREVIEWER = {Matthew Stover},
	DOI = {10.1007/s00039-014-0263-x},
	URL = {https://doi.org/10.1007/s00039-014-0263-x},
}
@article {lam-group-ext,
	AUTHOR = {Mitra, M.},
	TITLE = {Ending laminations for hyperbolic group extensions},
	JOURNAL = {Geom. Funct. Anal.},
	FJOURNAL = {Geometric and Functional Analysis},
	VOLUME = {7},
	YEAR = {1997},
	NUMBER = {2},
	PAGES = {379--402},
	ISSN = {1016-443X},
	MRCLASS = {20F32 (57M07)},
	MRNUMBER = {1445392},
	MRREVIEWER = {John Meier},
	DOI = {10.1007/PL00001624},
	URL = {https://doi.org/10.1007/PL00001624},
}
@article {dahmani,
	AUTHOR = {Dahmani, Fran\c{c}ois},
	TITLE = {Combination of convergence groups},
	JOURNAL = {Geom. Topol.},
	FJOURNAL = {Geometry and Topology},
	VOLUME = {7},
	YEAR = {2003},
	PAGES = {933--963},
	ISSN = {1465-3060},
	MRCLASS = {20F67 (20E06)},
	MRNUMBER = {2026551},
	DOI = {10.2140/gt.2003.7.933},
	URL = {https://doi.org/10.2140/gt.2003.7.933},
}
@article {ravi-1,
	AUTHOR = {Tomar, Ravi},
	TITLE = {Boundaries of graphs of relatively hyperbolic groups with cyclic edge groups.},
	URL = {https://arxiv.org/abs/2104.08843v1},
}
@article {mgrs,
	AUTHOR = {Gitik, Rita and Mitra, Mahan and Rips, Eliyahu and Sageev,
		Michah},
	TITLE = {Widths of subgroups},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {350},
	YEAR = {1998},
	NUMBER = {1},
	PAGES = {321--329},
	ISSN = {0002-9947},
	MRCLASS = {20F32 (57M07)},
	MRNUMBER = {1389776},
	MRREVIEWER = {Athanase Papadopoulos},
	DOI = {10.1090/S0002-9947-98-01792-9},
	URL = {https://doi.org/10.1090/S0002-9947-98-01792-9},
}
@article {mj-height,
	AUTHOR = {Mitra, Mahan},
	TITLE = {Height in splittings of hyperbolic groups},
	JOURNAL = {Proc. Indian Acad. Sci. Math. Sci.},
	FJOURNAL = {Indian Academy of Sciences. Proceedings. Mathematical
		Sciences},
	VOLUME = {114},
	YEAR = {2004},
	NUMBER = {1},
	PAGES = {39--54},
	ISSN = {0253-4142},
	MRCLASS = {20F67 (20E06 20F34)},
	MRNUMBER = {2040599},
	MRREVIEWER = {Denis V. Osin},
	DOI = {10.1007/BF02829670},
	URL = {https://doi.org/10.1007/BF02829670},
}
@article {twisted conjugacy,
	AUTHOR = {Fel'shtyn, Alexander and Gon\c{c}alves, Daciberg L.},
	TITLE = {Twisted conjugacy classes in symplectic groups, mapping class
		groups and braid groups},
	NOTE = {With an appendix written jointly with Francois Dahmani},
	JOURNAL = {Geom. Dedicata},
	FJOURNAL = {Geometriae Dedicata},
	VOLUME = {146},
	YEAR = {2010},
	PAGES = {211--223},
	ISSN = {0046-5755},
	MRCLASS = {20E45 (20F36 20F65 20G30 37C25 55M20 57M20)},
	MRNUMBER = {2644279},
	MRREVIEWER = {Darryl McCullough},
	DOI = {10.1007/s10711-009-9434-6},
	URL = {https://doi.org/10.1007/s10711-009-9434-6},
}
@book {serre,
	AUTHOR = {Serre, Jean-Pierre},
	TITLE = {Trees},
	SERIES = {Springer Monographs in Mathematics},
	NOTE = {Translated from the French original by John Stillwell,
		Corrected 2nd printing of the 1980 English translation},
	PUBLISHER = {Springer-Verlag, Berlin},
	YEAR = {2003},
	PAGES = {x+142},
	ISBN = {3-540-44237-5},
	MRCLASS = {20E08 (05C05 20E06 20G25)},
	MRNUMBER = {1954121},
}
@article {SK-1,
	AUTHOR = {Krishna, Swathi},
	TITLE = {Relatively hyperbolic metric bundles and Cannon-Thurston maps},
	note = {\url{https://arxiv.org/pdf/2204.01073.pdf}},
}
@article {SBSK,
	AUTHOR = {Bhunia, Sushil and Krishna, Swathi},
	TITLE = {Twisted conjugacy in big mapping class groups},
	JOURNAL = {Topology Appl.},
	FJOURNAL = {Topology and its Applications},
	VOLUME = {324},
	YEAR = {2023},
	PAGES = {Paper No. 108353, 13},
	ISSN = {0166-8641,1879-3207},
	MRCLASS = {20E45 (20F65 57M07)},
	MRNUMBER = {4525669},
	MRREVIEWER = {Egle\ Bettio},
	DOI = {10.1016/j.topol.2022.108353},
	URL = {https://doi.org/10.1016/j.topol.2022.108353},
}
@article {Itai,
	AUTHOR = {Benjamini, Itai and Tessera, Romain},
	TITLE = {First passage percolation on a hyperbolic graph admits
		bi-infinite geodesics},
	JOURNAL = {Electron. Commun. Probab.},
	FJOURNAL = {Electronic Communications in Probability},
	VOLUME = {22},
	YEAR = {2017},
	PAGES = {Paper No. 14, 8},
	MRCLASS = {82B43 (60D05)},
	MRNUMBER = {3615665},
	DOI = {10.1214/17-ECP44},
	URL = {https://doi.org/10.1214/17-ECP44},
}
@article {mjbasu,
	AUTHOR = {Basu, Riddhipratim and Mj, Mahan},
	TITLE = {First passage percolation on hyperbolic groups},
	JOURNAL = {Preprint},
	URL = {https://arxiv.org/abs/1909.03427},
	YEAR= {2019},
}
}
@article {jpmutanguha,
AUTHOR = {Mutanguha, Jean Pierre},
TITLE = {The dynamics and geometry of free group endomorphisms},
JOURNAL = {Adv. Math.},
FJOURNAL = {Advances in Mathematics},
VOLUME = {384},
YEAR = {2021},
PAGES = {Paper No. 107714, 60},
ISSN = {0001-8708,1090-2082},
MRCLASS = {20E05 (20E06 20E36)},
MRNUMBER = {4237417},
MRREVIEWER = {Anthony\ Genevois},
DOI = {10.1016/j.aim.2021.107714},
URL = {https://doi.org/10.1016/j.aim.2021.107714},
}

@article {JPMrel,
AUTHOR = {Mutanguha, Jean Pierre},
TITLE = {Irreducibility of a free group endomorphism is a mapping torus
	invariant},
JOURNAL = {Comment. Math. Helv.},
FJOURNAL = {Commentarii Mathematici Helvetici. A Journal of the Swiss
	Mathematical Society},
VOLUME = {96},
YEAR = {2021},
NUMBER = {1},
PAGES = {47--63},
ISSN = {0010-2571,1420-8946},
MRCLASS = {20F65 (20E05 20E06 20F67)},
MRNUMBER = {4228613},
MRREVIEWER = {Sushil\ Bhunia},
DOI = {10.4171/cmh/506},
URL = {https://doi.org/10.4171/cmh/506},
}

@article {JPMhyperbolic,
AUTHOR = {Mutanguha, Jean Pierre},
TITLE = {Hyperbolic immersions of free groups},
JOURNAL = {Groups Geom. Dyn.},
FJOURNAL = {Groups, Geometry, and Dynamics},
VOLUME = {14},
YEAR = {2020},
NUMBER = {4},
PAGES = {1253--1275},
ISSN = {1661-7207,1661-7215},
MRCLASS = {20F65 (20E05 20F67)},
MRNUMBER = {4186474},
MRREVIEWER = {J.\ S.\ Birman},
DOI = {10.4171/ggd/580},
URL = {https://doi.org/10.4171/ggd/580},
}

@article {JPMnonsurj,
AUTHOR = {Mutanguha, Jean Pierre},
TITLE = {Irreducible nonsurjective endomorphisms of {$F_n$} are
	hyperbolic},
JOURNAL = {Bull. Lond. Math. Soc.},
FJOURNAL = {Bulletin of the London Mathematical Society},
VOLUME = {52},
YEAR = {2020},
NUMBER = {5},
PAGES = {960--976},
ISSN = {0024-6093,1469-2120},
MRCLASS = {20F67 (20E05 20E08 20F65)},
MRNUMBER = {4171415},
MRREVIEWER = {Thomas\ Koberda},
DOI = {10.1112/blms.12377},
URL = {https://doi.org/10.1112/blms.12377},
}
@book {JPM,
AUTHOR = {Mutanguha, Jean Pierre},
TITLE = {Hyperbolic {E}ndomorphisms of {F}ree {G}roups},
NOTE = {Thesis (Ph.D.)--University of Arkansas},
PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
YEAR = {2020},
PAGES = {78},
ISBN = {979-8643-19925-0},
MRCLASS = {99-05},
MRNUMBER = {4106375},
URL =
{http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqm&rft_dat=xri:pqdiss:27837244},
}
@article {IKendo,
AUTHOR = {Kapovich, Ilya},
TITLE = {Mapping tori of endomorphisms of free groups},
JOURNAL = {Comm. Algebra},
FJOURNAL = {Communications in Algebra},
VOLUME = {28},
YEAR = {2000},
NUMBER = {6},
PAGES = {2895--2917},
ISSN = {0092-7872,1532-4125},
MRCLASS = {20F67 (20E05 20E06 57M07)},
MRNUMBER = {1757436},
MRREVIEWER = {S.\ Andreadakis},
DOI = {10.1080/00927870008826999},
URL = {https://doi.org/10.1080/00927870008826999},
}
@article {DahmaniLi,
AUTHOR = {Dahmani, Fran\c{c}ois and Li, Ruoyu},
TITLE = {Relative hyperbolicity for automorphisms of free products and
	free groups},
JOURNAL = {J. Topol. Anal.},
FJOURNAL = {Journal of Topology and Analysis},
VOLUME = {14},
YEAR = {2022},
NUMBER = {1},
PAGES = {55--92},
ISSN = {1793-5253,1793-7167},
MRCLASS = {20F67 (20F34 20F65)},
MRNUMBER = {4411100},
MRREVIEWER = {Thomas\ Koberda},
DOI = {10.1142/S1793525321500011},
URL = {https://doi.org/10.1142/S1793525321500011},
}
@article {brinkmann,
AUTHOR = {Brinkmann, P.},
TITLE = {Hyperbolic automorphisms of free groups},
JOURNAL = {Geom. Funct. Anal.},
FJOURNAL = {Geometric and Functional Analysis},
VOLUME = {10},
YEAR = {2000},
NUMBER = {5},
PAGES = {1071--1089},
ISSN = {1016-443X,1420-8970},
MRCLASS = {20F65 (20E36 57M07)},
MRNUMBER = {1800064},
MRREVIEWER = {Katalin\ A.\ Bencsath},
DOI = {10.1007/PL00001647},
URL = {https://doi.org/10.1007/PL00001647},
}
@article {pritam,
AUTHOR = {Ghosh, Pritam},
TITLE = {Relative hyperbolicity of free-by-cyclic extensions},
JOURNAL = {Compos. Math.},
FJOURNAL = {Compositio Mathematica},
VOLUME = {159},
YEAR = {2023},
NUMBER = {1},
PAGES = {153--183},
ISSN = {0010-437X,1570-5846},
MRCLASS = {20F65 (20E05 20F67 57M07)},
MRNUMBER = {4541452},
MRREVIEWER = {Anthony\ Genevois},
DOI = {10.1112/S0010437X22007813},
URL = {https://doi.org/10.1112/S0010437X22007813},
}
@article {mitscottswarup,
AUTHOR = {Mitra, Mahan},
TITLE = {On a theorem of {S}cott and {S}warup},
JOURNAL = {Proc. Amer. Math. Soc.},
FJOURNAL = {Proceedings of the American Mathematical Society},
VOLUME = {127},
YEAR = {1999},
NUMBER = {6},
PAGES = {1625--1631},
ISSN = {0002-9939,1088-6826},
MRCLASS = {20F32 (57M50 57N10)},
MRNUMBER = {1610757},
MRREVIEWER = {Dubravko\ Ivan\v{s}i\'{c}},
DOI = {10.1090/S0002-9939-99-04935-7},
URL = {https://doi.org/10.1090/S0002-9939-99-04935-7},
}
@article {mj2009,
AUTHOR = {Mj, Mahan},
TITLE = {Cannon-{T}hurston maps for pared manifolds of bounded
	geometry},
JOURNAL = {Geom. Topol.},
FJOURNAL = {Geometry \& Topology},
VOLUME = {13},
YEAR = {2009},
NUMBER = {1},
PAGES = {189--245},
ISSN = {1465-3060,1364-0380},
MRCLASS = {57M50},
MRNUMBER = {2469517},
MRREVIEWER = {Vassilis\ Metaftsis},
DOI = {10.2140/gt.2009.13.189},
URL = {https://doi.org/10.2140/gt.2009.13.189},
}

@incollection {mj2010,
AUTHOR = {Mj, Mahan},
TITLE = {Cannon-{T}hurston maps and bounded geometry},
BOOKTITLE = {Teichm\"{u}ller theory and moduli problem},
SERIES = {Ramanujan Math. Soc. Lect. Notes Ser.},
VOLUME = {10},
PAGES = {489--511},
PUBLISHER = {Ramanujan Math. Soc., Mysore},
YEAR = {2010},
ISBN = {978-93-80416-00-7},
MRCLASS = {20F65 (57M50)},
MRNUMBER = {2667569},
MRREVIEWER = {Thomas\ Koberda},
}
@incollection {mj2016,
AUTHOR = {Mj, Mahan},
TITLE = {Cannon-{T}hurston maps for surface groups: an exposition of
	amalgamation geometry and split geometry},
BOOKTITLE = {Geometry, topology, and dynamics in negative curvature},
SERIES = {London Math. Soc. Lecture Note Ser.},
VOLUME = {425},
PAGES = {221--271},
PUBLISHER = {Cambridge Univ. Press, Cambridge},
YEAR = {2016},
ISBN = {978-1-107-52900-7},
MRCLASS = {57M50 (57M05)},
MRNUMBER = {3497262},
MRREVIEWER = {Baris\ Coskunuzer},
}
@article {Pat,
AUTHOR = {Reynolds, Patrick.},
TITLE = {DYNAMICS OF IRREDUCIBLE ENDOMORPHISMS OF Fn.},
URL = {https://arxiv.org/pdf/1008.3659.pdf},
}
@article {gaboriau,
AUTHOR = {Gaboriau, Damien and Jaeger, Andre and Levitt, Gilbert and
	Lustig, Martin},
TITLE = {An index for counting fixed points of automorphisms of free
	groups},
JOURNAL = {Duke Math. J.},
FJOURNAL = {Duke Mathematical Journal},
VOLUME = {93},
YEAR = {1998},
NUMBER = {3},
PAGES = {425--452},
ISSN = {0012-7094,1547-7398},
MRCLASS = {20E36 (20E05 20E08 57M07)},
MRNUMBER = {1626723},
MRREVIEWER = {Olympia\ Talelli},
DOI = {10.1215/S0012-7094-98-09314-0},
URL = {https://doi.org/10.1215/S0012-7094-98-09314-0},
}
@article {wisebigdley,
AUTHOR = {Bigdely, Hadi and Wise, Daniel T.},
TITLE = {Quasiconvexity and relatively hyperbolic groups that split},
JOURNAL = {Michigan Math. J.},
FJOURNAL = {Michigan Mathematical Journal},
VOLUME = {62},
YEAR = {2013},
NUMBER = {2},
PAGES = {387--406},
ISSN = {0026-2285,1945-2365},
MRCLASS = {20F67 (20F65)},
MRNUMBER = {3079269},
MRREVIEWER = {Mahan\ Mj},
DOI = {10.1307/mmj/1370870378},
URL = {https://doi.org/10.1307/mmj/1370870378},
}
@article {gl-outer,
AUTHOR = {Guirardel, Vincent and Levitt, Gilbert},
TITLE = {The outer space of a free product},
JOURNAL = {Proc. Lond. Math. Soc. (3)},
FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
VOLUME = {94},
YEAR = {2007},
NUMBER = {3},
PAGES = {695--714},
ISSN = {0024-6115,1460-244X},
MRCLASS = {20E06 (20E08 20F28 20F65)},
MRNUMBER = {2325317},
MRREVIEWER = {Dimitrios\ Varsos},
DOI = {10.1112/plms/pdl026},
URL = {https://doi.org/10.1112/plms/pdl026},
}
@article {FranMartino,
AUTHOR = {Francaviglia, Stefano and Martino, Armando},
TITLE = {Stretching factors, metrics and train tracks for free
	products},
JOURNAL = {Illinois J. Math.},
FJOURNAL = {Illinois Journal of Mathematics},
VOLUME = {59},
YEAR = {2015},
NUMBER = {4},
PAGES = {859--899},
ISSN = {0019-2082,1945-6581},
MRCLASS = {20E08 (20E06 20E36 20F65)},
MRNUMBER = {3628293},
MRREVIEWER = {Mihalis\ A.\ Sykiotis},
URL = {http://projecteuclid.org/euclid.ijm/1488186013},
}
@article {CM,
AUTHOR = {Culler, Marc and Morgan, John W.},
TITLE = {Group actions on {${\bf R}$}-trees},
JOURNAL = {Proc. London Math. Soc. (3)},
FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
VOLUME = {55},
YEAR = {1987},
NUMBER = {3},
PAGES = {571--604},
ISSN = {0024-6115,1460-244X},
MRCLASS = {20F32 (57N10)},
MRNUMBER = {907233},
MRREVIEWER = {Roger\ C.\ Alperin},
DOI = {10.1112/plms/s3-55.3.571},
URL = {https://doi.org/10.1112/plms/s3-55.3.571},
}
@article {bowditch-relhyp,
AUTHOR = {Bowditch, B. H.},
TITLE = {Relatively hyperbolic groups},
JOURNAL = {Internat. J. Algebra Comput.},
FJOURNAL = {International Journal of Algebra and Computation},
VOLUME = {22},
YEAR = {2012},
NUMBER = {3},
PAGES = {1250016, 66},
ISSN = {0218-1967,1793-6500},
MRCLASS = {20F67 (20F65)},
MRNUMBER = {2922380},
MRREVIEWER = {R\'{e}mi\ Bernard\ Coulon},
DOI = {10.1142/S0218196712500166},
URL = {https://doi.org/10.1142/S0218196712500166},
}
@article {horbez,
AUTHOR = {Horbez, Camille},
TITLE = {The boundary of the outer space of a free product},
JOURNAL = {Israel J. Math.},
FJOURNAL = {Israel Journal of Mathematics},
VOLUME = {221},
YEAR = {2017},
NUMBER = {1},
PAGES = {179--234},
ISSN = {0021-2172,1565-8511},
MRCLASS = {20F65 (05C05 05C25 20E06 57M07)},
MRNUMBER = {3705852},
MRREVIEWER = {Funda\ G\"{u}ltepe},
DOI = {10.1007/s11856-017-1565-0},
URL = {https://doi.org/10.1007/s11856-017-1565-0},
}
@article {farb,
AUTHOR = {Farb, B.},
TITLE = {Relatively hyperbolic groups},
JOURNAL = {Geom. Funct. Anal.},
FJOURNAL = {Geometric and Functional Analysis},
VOLUME = {8},
YEAR = {1998},
NUMBER = {5},
PAGES = {810--840},
ISSN = {1016-443X,1420-8970},
MRCLASS = {20F32 (20F10 57M07)},
MRNUMBER = {1650094},
MRREVIEWER = {Michel\ Coornaert},
DOI = {10.1007/s000390050075},
URL = {https://doi.org/10.1007/s000390050075},
}
@article {groves-manning,
AUTHOR = {Groves, Daniel and Manning, Jason Fox},
TITLE = {Dehn filling in relatively hyperbolic groups},
JOURNAL = {Israel J. Math.},
FJOURNAL = {Israel Journal of Mathematics},
VOLUME = {168},
YEAR = {2008},
PAGES = {317--429},
ISSN = {0021-2172,1565-8511},
MRCLASS = {57M50},
MRNUMBER = {2448064},
MRREVIEWER = {Colin\ C.\ Adams},
DOI = {10.1007/s11856-008-1070-6},
URL = {https://doi.org/10.1007/s11856-008-1070-6},
}
@article {traintrack,
AUTHOR = {Bestvina, Mladen and Handel, Michael},
TITLE = {Train tracks and automorphisms of free groups},
JOURNAL = {Ann. of Math. (2)},
FJOURNAL = {Annals of Mathematics. Second Series},
VOLUME = {135},
YEAR = {1992},
NUMBER = {1},
PAGES = {1--51},
ISSN = {0003-486X,1939-8980},
MRCLASS = {20E05 (20F28 20F32 20F34 57M07 57M15)},
MRNUMBER = {1147956},
MRREVIEWER = {Darryl\ McCullough},
DOI = {10.2307/2946562},
URL = {https://doi.org/10.2307/2946562},
}
@article {MCML,
AUTHOR = {Cohen, Marshall M. and Lustig, Martin},
TITLE = {Very small group actions on {${\bf R}$}-trees and {D}ehn twist
	automorphisms},
JOURNAL = {Topology},
FJOURNAL = {Topology. An International Journal of Mathematics},
VOLUME = {34},
YEAR = {1995},
NUMBER = {3},
PAGES = {575--617},
ISSN = {0040-9383},
MRCLASS = {20F32 (20E05 20E08 20F28)},
MRNUMBER = {1341810},
MRREVIEWER = {Gilbert\ Levitt},
DOI = {10.1016/0040-9383(94)00038-M},
URL = {https://doi.org/10.1016/0040-9383(94)00038-M},
}
@article {kbutton,
AUTHOR = {Button, J. O. and Kropholler, R. P.},
TITLE = {Nonhyperbolic free-by-cyclic and one-relator groups},
JOURNAL = {New York J. Math.},
FJOURNAL = {New York Journal of Mathematics},
VOLUME = {22},
YEAR = {2016},
PAGES = {755--774},
ISSN = {1076-9803},
MRCLASS = {20F67 (20E22 20F05 57M20)},
MRNUMBER = {3548122},
MRREVIEWER = {R\'emi\ Bernard\ Coulon},
URL = {http://nyjm.albany.edu:8000/j/2016/22_755.html},
}
@article {FH-coherent,
AUTHOR = {Feighn, Mark and Handel, Michael},
TITLE = {Mapping tori of free group automorphisms are coherent},
JOURNAL = {Ann. of Math. (2)},
FJOURNAL = {Annals of Mathematics. Second Series},
VOLUME = {149},
YEAR = {1999},
NUMBER = {3},
PAGES = {1061--1077},
ISSN = {0003-486X,1939-8980},
MRCLASS = {20F05 (20E06 20F34 57M07)},
MRNUMBER = {1709311},
MRREVIEWER = {Michael\ L.\ Mihalik},
DOI = {10.2307/121081},
URL = {https://doi.org/10.2307/121081},
}
@book {bieri,
AUTHOR = {Bieri, Robert},
TITLE = {Homological dimension of discrete groups},
SERIES = {Queen Mary College Mathematics Notes},
EDITION = {Second},
PUBLISHER = {Queen Mary College, Department of Pure Mathematics, London},
YEAR = {1981},
PAGES = {iv+198},
MRCLASS = {20J05 (18G20 57P10)},
MRNUMBER = {715779},
}
@article {JPMrelhyp,
AUTHOR = {Mutanguha, Jean Pierre},
TITLE = {Relative expansions for free group endomorphisms},
URL = {https://mutanguha.com/pdfs/survey.pdf},
YEAR= {2024},
}
@incollection {gersten,
AUTHOR = {Gersten, S. M.},
TITLE = {Dehn functions and {$l_1$}-norms of finite presentations},
BOOKTITLE = {Algorithms and classification in combinatorial group theory
	({B}erkeley, {CA}, 1989)},
SERIES = {Math. Sci. Res. Inst. Publ.},
VOLUME = {23},
PAGES = {195--224},
PUBLISHER = {Springer, New York},
YEAR = {1992},
ISBN = {0-387-97685-X},
MRCLASS = {20F32 (57M07)},
MRNUMBER = {1230635},
MRREVIEWER = {W.\ Metzler and Stephan\ Rosebrock},
DOI = {10.1007/978-1-4613-9730-4\_9},
URL = {https://doi.org/10.1007/978-1-4613-9730-4_9},
}
@article {groves-herm,
AUTHOR = {Groves, J. R. J. and Hermiller, S. M.},
TITLE = {Isoperimetric inequalities for soluble groups},
JOURNAL = {Geom. Dedicata},
FJOURNAL = {Geometriae Dedicata},
VOLUME = {88},
YEAR = {2001},
NUMBER = {1-3},
PAGES = {239--254},
ISSN = {0046-5755,1572-9168},
MRCLASS = {20F65 (20E06)},
MRNUMBER = {1877218},
MRREVIEWER = {Stephen\ G.\ Brick},
DOI = {10.1023/A:1013110821237},
URL = {https://doi.org/10.1023/A:1013110821237},
}
@article {MBDG,
AUTHOR = {Bridson, Martin R. and Groves, Daniel},
TITLE = {The quadratic isoperimetric inequality for mapping tori of
	free group automorphisms},
JOURNAL = {Mem. Amer. Math. Soc.},
FJOURNAL = {Memoirs of the American Mathematical Society},
VOLUME = {203},
YEAR = {2010},
NUMBER = {955},
PAGES = {xii+152},
ISSN = {0065-9266,1947-6221},
ISBN = {978-0-8218-4631-5},
MRCLASS = {20F65 (20E36 20F06 57M07)},
MRNUMBER = {2590896},
MRREVIEWER = {Ian\ M.\ Chiswell},
DOI = {10.1090/S0065-9266-09-00578-X},
URL = {https://doi.org/10.1090/S0065-9266-09-00578-X},
}
@article {DS-RD,
AUTHOR = {Dru\c tu, Cornelia and Sapir, Mark},
TITLE = {Relatively hyperbolic groups with rapid decay property},
JOURNAL = {Int. Math. Res. Not.},
FJOURNAL = {International Mathematics Research Notices},
YEAR = {2005},
NUMBER = {19},
PAGES = {1181--1194},
ISSN = {1073-7928,1687-0247},
MRCLASS = {20F67},
MRNUMBER = {2147058},
MRREVIEWER = {Paul\ D.\ Mitchener},
DOI = {10.1155/IMRN.2005.1181},
URL = {https://doi.org/10.1155/IMRN.2005.1181},
}
@article {surajdahmani,
AUTHOR = {Dahmani, Fran\c cois and Krishna M S, Suraj},
TITLE = {Relative hyperbolicity of hyperbolic-by-cyclic groups},
JOURNAL = {Groups Geom. Dyn.},
FJOURNAL = {Groups, Geometry, and Dynamics},
VOLUME = {17},
YEAR = {2023},
NUMBER = {2},
PAGES = {403--426},
ISSN = {1661-7207,1661-7215},
MRCLASS = {20F65 (20E08 20E36 20F67)},
MRNUMBER = {4584670},
MRREVIEWER = {John\ M.\ Mackay},
DOI = {10.4171/ggd/703},
URL = {https://doi.org/10.4171/ggd/703},
}
@incollection {chatterji-rdp,
AUTHOR = {Chatterji, Indira},
TITLE = {Introduction to the rapid decay property},
BOOKTITLE = {Around {L}anglands correspondences},
SERIES = {Contemp. Math.},
VOLUME = {691},
PAGES = {53--72},
PUBLISHER = {Amer. Math. Soc., Providence, RI},
YEAR = {2017},
ISBN = {978-1-4704-3573-8},
MRCLASS = {20-02 (20F65 22D40)},
MRNUMBER = {3666050},
DOI = {10.1090/conm/691/13893},
URL = {https://doi.org/10.1090/conm/691/13893},
}
@article {jolis-hyp,
AUTHOR = {Jolissaint, Paul},
TITLE = {Rapidly decreasing functions in reduced {$C^*$}-algebras of
	groups},
JOURNAL = {Trans. Amer. Math. Soc.},
FJOURNAL = {Transactions of the American Mathematical Society},
VOLUME = {317},
YEAR = {1990},
NUMBER = {1},
PAGES = {167--196},
ISSN = {0002-9947,1088-6850},
MRCLASS = {22D25 (43A15 46L99)},
MRNUMBER = {943303},
MRREVIEWER = {A.\ Derighetti},
DOI = {10.2307/2001458},
URL = {https://doi.org/10.2307/2001458},
}
@article {rdp-hyp,
AUTHOR = {de la Harpe, Pierre},
TITLE = {Groupes hyperboliques, alg\`ebres d'op\'erateurs et un
	th\'eor\`eme de {J}olissaint},
JOURNAL = {C. R. Acad. Sci. Paris S\'er. I Math.},
FJOURNAL = {Comptes Rendus des S\'eances de l'Acad\'emie des Sciences.
	S\'erie I. Math\'ematique},
VOLUME = {307},
YEAR = {1988},
NUMBER = {14},
PAGES = {771--774},
ISSN = {0249-6291},
MRCLASS = {22D25 (20F38 22E40 46L80 58G12)},
MRNUMBER = {972078},
MRREVIEWER = {Alain\ Valette},
}
@article {rdp-relhyp,
AUTHOR = {Dru\c tu, Cornelia and Sapir, Mark},
TITLE = {Relatively hyperbolic groups with rapid decay property},
JOURNAL = {Int. Math. Res. Not.},
FJOURNAL = {International Mathematics Research Notices},
YEAR = {2005},
NUMBER = {19},
PAGES = {1181--1194},
ISSN = {1073-7928,1687-0247},
MRCLASS = {20F67},
MRNUMBER = {2147058},
MRREVIEWER = {Paul\ D.\ Mitchener},
DOI = {10.1155/IMRN.2005.1181},
URL = {https://doi.org/10.1155/IMRN.2005.1181},
}
@article {gautero-lustig-rdp,
AUTHOR = {Gautero, Fran\c cois and Lustig, Martin},
TITLE = {The mapping torus group of a free group automorphism is hyperbolic relative to the canonical subgroups of polynomial growth},
URL = {https://doi.org/10.48550/arXiv.0707.0822},
}


